SFC: Near-Source Congestion Signaling and Flow Control

State-of-the-art congestion control algorithms for data centers alone do not cope well with transient congestion and high traffic bursts. To help with these, we revisit the concept of direct \emph{backward} feedback from switches and propose Back-to-Sender (BTS) signaling to many concurrent incast senders. Combining it with our novel approach to in-network caching, we achieve near-source sub-RTT congestion signaling. Source Flow Control (SFC) combines these two simple signaling mechanisms to instantly pause traffic sources, hence avoiding the head-of-line blocking problem of conventional hop-by-hop flow control. Our prototype system and scale simulations demonstrate that near-source signaling can significantly reduce the message completion time of various workloads in the presence of incast, complementing existing congestion control algorithms. Our results show that SFC can reduce the $99^{th}$-percentile flow completion times by $1.2-6\times$ and the peak switch buffer usage by $2-3\times$ compared to the recent incast solutions.

==> Makefile <==
#
# $Id: Makefile,v 1.1 2006/06/27 21:10:04 shafer Exp $
#
# Makefile for converting tex files to PDF
#

PAPER = main

# directories
OUTPUT_DIR = ./
BIB_OUT_FILE = bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR):$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(PAPER).log | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat *.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)
PRINT_BIBTEX_NOTE = if [ -s $(BIB_OUT_FILE) ]; then \
                    echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."; fi


all: $(PAPER).pdf

#
# We want our main "pdf" to depend on all the "tex" and "bib" source
#

#main.pdf: sig-alternate-10pt.cls *.tex *.bib figures/*
#main.pdf: acmart.cls *.tex *.bib figures/*

main.pdf: *.tex *.bib  
#
# Now provide the rules for building the various targets and
# intermediate targets
#

%.pdf : %.tex
	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS) $(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi
	@-$(PRINT_BIBTEX_WARNINGS)
	@-$(PRINT_BIBTEX_NOTE)


	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)


	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)


%.ps : %.dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -j0 -o $@ $<

# %.pdf : %.ps
# 	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dCompatibilityLevel=1.2 -dProcessColorModel=/DeviceGray -dSubsetFonts=true -dMaxSubsetPct=100 $< $@

clean:
	-rm -f *.dvi *.log *.aux *.bbl *.blg *.ent *.out main.pdf

#
# Run "make balance" after adding balance columns at the right place
#

balance:
	latex main
	latex main
	dvips -o main.ps main.dvi
	ps2pdf main.ps main.pdf


==> sections/___6related.tex <==

\section{Related Work}
\label{sec:related}

Our work draws on the long history of congestion control (CC) and flow
control (FC) mechanisms, many of which were mentioned
previously. Below we outline additional work closely related to BTS
and \sys.

\paragraph*{Backward Switch Feedback.}
%
We acknowledge that prior work has proposed backward notifications
from switches. However, they were not widely adopted for various
reasons.  ICMP Source Quench~\cite{icmp} was proposed for the Internet
CC, but officially deprecated from the IETF because: (1) it lacked a
clear specification of how senders should react to the quench, and (2)
there was a lack of trust between devices in WAN.
BECN~\cite{newman93,newman94} was another early proposal; it is tied
to specific congestion signal (ECN) and requires the 1st RTT packets
to be ACK'ed by the receiver first to mark ECN on them, hence does not
enable sub-RTT signaling.  QCN~\cite{alizadeh08} is similar to SFC as
it implements pre-queuing congestion detection and backward
notification.  QCN as an L2 CC scheme was not widely deployed in L3
data centers and is not applicable to L4 RDMA transport protocols.

%FastLane~\cite{fastlane} uses direct loss notification from switches.
%It demonstrated reduced FCT for TCP using simulations.

As a recent proposal, Annulus~\cite{annulus} uses switch direct
feedback to mitigate high-RTT WAN traffic penalizing low-RTT
datacenter traffic. Annulus uses the L2 MAC learning feature to
generate backward feedback as a short-term prototype and
\emph{"presents a motivation for developing schemes that can report
INT signals directly to sender from switches"} for better near-source
control loops.  NDP~\cite{ndp} employs cut-payload trimming to shorten
the incast signaling delay in the receiver-driven CC architecture.
Trimming cannot cope with extremely large incast and works only at the
last-hop ToR switch. NDP discussed Return-to-Sender (RTS) as an
optimization idea without a system design and limited to the
receiver-driven architecture.  BTS is our answer for generic backward
signaling from switches.  We provide a concrete system design and
present SFC as a new multi-hop flow control(FC) use case of backward signaling.

\paragraph*{Flow Control.}
%
%Like \sys, IRN~\cite{irn} seeks an alternative to PFC for RDMA. IRN
%uses a fixed-sized window for flow control and selective
%retransmission for loss recovery.  In general, selective
%retransmission requires more complex algorithms and buffer management
%in the end-host NICs. A simple switch-side assistance like SN*
%achieves a comparable performance and works with standard RDMA NICs.

Due to its fast reaction and simplicity, FC has received a renewed
attention for replacing end-to-end CC (e.g., BFC~\cite{bfc}) or augmenting it
(e.g., OnRamp~\cite{onramp}).  BFC aims to fully replace end-to-end CC by
per-flow back-pressure up to the traffic sources. Atop the BFC
discussion in~\S\ref{sub:bts-limit}, BFC needs the entire network
(switches and NICs) to be upgraded at once.  In contrast, \sys pauses
traffic at the source directly and allows brown field deployments
starting from enabling it on ToR switches only. OnRamp employs a FC as
a faster reaction (than CC) to incast and transient congestion but
still uses end-to-end signaling loop coupled with the congestion.  In
addition, while being more precise than RTT, the one-way delay signal
of OnRamp reflects the past congestion experienced by packets at
network egress rather than the currently expected queueing time we use
in BTS.

%%%CP~\cite{cp} and NDP~\cite{ndp} use cut-payload schemes to signal
%%%congestion and loss events to the receiver. Cut-payload schemes can slow
%%%the transmission down to some degree because it consumes bandwidth of the
%%%bottleneck link.  \sys borrows this concept for SN* but without
%%%prioritizing the truncated packets.  We argue that direct backward feedback
%%%(like SN) offers a better solution, since it avoids interruption on
%%%the bottleneck link. In general, receiver-driven approaches~\cite{ndp,
%%%  homa} have a limitation in handling network core congestion.
%%%
%%%RDMA Receiver-Not-Ready (RNR) NAKs are a combination of pause and NAK messages.
%%%%This combination helps to reduce PPS overhead at the NIC resources.
%%%They are designed to react to receiver NIC bottlenecks,
%%%not to help with switch buffer depletion. The pause time resolution is too
%%%coarse-grained to achieve low-latency retransmission.


==> sections/removed_figures.tex <==
\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 10
    \centering
    \includegraphics{plots/fig10b_dcqcn_rev.pdf} %fig10_aggr_med.pdf
    \caption{{\bf RPC} workload with 30\% load + 5\% 128-to-1 incast and with {\it \bf DCQCN+W} as
        congestion control algorithm.
        {\bf GBN, IRN, PFC, Onramp+IRN, Onramp+PFC, SFC+GBN}, drop P50, only present P95, P99, P99.99.  } %#, SFC+IRN
    \label{fig:w3-30-}
    \end{minipage}   
    \vspace{-0.2in}
\end{figure*}
\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 10
    \centering
    \includegraphics{plots/fig10b_hpcc_rev.pdf} %fig10_aggr_med.pdf
    \caption{{\bf RPC} workload with 30\% load + 5\% 128-to-1 incastand with {\it \bf HPCC} as
        congestion control algorithm.}
    \label{fig:w3-30-}
    \end{minipage}   
    \vspace{-0.2in}
\end{figure*}

\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 10
    \centering
    \includegraphics{plots/fig10_dcqcn_rev.pdf} %fig10_aggr_med.pdf
    \caption{{\bf Hadoop} workload with 50\% load without incast and with {\it \bf DCQCN+W} as
        congestion control algorithm.}
    \label{fig:w3-30-}
    \end{minipage}   
    \vspace{-0.2in}
\end{figure*}
\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 10
    \centering
    \includegraphics{plots/fig10_hpcc_rev.pdf} %fig10_aggr_med.pdf
    \caption{{\bf Hadoop} workload with 50\% load without incast and with {\it \bf HPCC} as
        congestion control algorithm.}
    \label{fig:w3-30-}
    \end{minipage}   
    \vspace{-0.2in}
\end{figure*}

\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 11
    \centering
    \includegraphics{plots/fig11_dcqcn_rev.pdf} %fig11_aggr_med.pdf
    \caption{{\bf Hadoop} workload with 50\% load + 5\% 128-to-1 incast with {\it \bf DCQCN} as congestion control algorithm.}
    \label{fig:w4-50-}
    \end{minipage}    
    \vspace{-0.15in}
\end{figure*}

\begin{figure*}[!htb]
\begin{minipage}{1.0\linewidth}
% Figure 11
    \centering
    \includegraphics{plots/fig11_hpcc_rev.pdf} %fig11_aggr_med.pdf
    \caption{{\bf Hadoop} workload with 50\% load + 5\% 128-to-1 incast with {\it \bf HPCC} as congestion control algorithm.
    Without incast, see how 80\% without incast + HPCC  }
    \label{fig:w4-50-}
    \end{minipage}    
    \vspace{-0.15in}
\end{figure*}

==> sections/sigcomm-outline.tex <==
\section{New Storyline for Sigcomm}

\begin{itemize}
  \item Context: same as before
  \item Problem: the same, but add implementational and operational complexity as issues
  \item Issues that SFC addresses
  \begin{itemize}
    \item Over QCN: handle incast better (stopping)
    \item Over QCN: as FC mechanism, can be combined with CC mechanism. We do FC, they do CC
    \item Operational complexity: Simple to implement (Computational and state complexity on switch and on NIC)
    \item Operational complexity: Easy to configure (Number of parameters and how to select them)
  \end{itemize}
  \item Key contributions and Novelty in SFC
  \begin{itemize}
    \item In-network feedback before queueing
    \item "the best possible way to signal and react to incast events"
    \item Options: Caching SFc?, Multicast SFC? Predictive SFC?
  \end{itemize}
\end{itemize}

New papers to cite:
\begin{itemize}
  \item Meta microburst paper: parallelism in congestion
  \item SRNIC?
  \item ABM?
  \item Poseidon (link delay setup)
  \item Bolt
  \item QCN companion paper
\end{itemize}


New settings/parameters
\begin{itemize}
  \item 
\end{itemize}


See \enquote{Storyline} todo boxes for per-chapter story line notes. Use the same command to add new todos.



